Flavor Physics in the Quark Sector

One of the major challenges of particle physics has been to gain an in-depth understanding of the role of quark flavor and measurements and theoretical interpretations of their results have advanced tremendously: apart from masses and quantum numbers of flavor particles, there now exist detailed measurements of the characteristics of their interactions allowing stringent tests of Standard Model predictions. Among the most interesting phenomena of flavor physics is the violation of the CP symmetry that has been subtle and difficult to explore. Till early 1990s observations of CP violation were confined to neutral $K$ mesons, but since then a large number of CP-violating processes have been studied in detail in neutral $B$ mesons. In parallel, measurements of the couplings of the heavy quarks and the dynamics for their decays in large samples of $K, D$, and $B$ mesons have been greatly improved in accuracy and the results are being used as probes in the search for deviations from the Standard Model. In the near future, there will be a transition from the current to a new generation of experiments, thus a review of the status of quark flavor physics is timely. This report summarizes the results of the current generation of experiments that is about to be completed and it confronts these results with the theoretical understanding of the field.

==> charm.tex <==
\section{Measurement of the CKM mtrix elements in $D$ decays[10 pages]}
\subsection{Semileptonic $D$ decays}
\subsubsection{ Measurement of \Vcs\ in Exclusive CKM-favored decays}
\subsubsubsection{Constraints on form factors}
\subsubsubsection{Form factors and branching fraction measurements}
\subsubsubsection{Determination of \Vcs}
\subsubsection{Exclusive CKM-suppressed decays}
\subsubsubsection{Form factors and branching fraction measurements}
\subsubsubsection{Determination of \Vcd}


==> mixPhase.tex <==
\section{Measurement of phases of the CKM matrix elements in tree-dominated processes [25 pages]}
\subsection{Measurements of the angle \bb in tree dominated processes}
\subsubsection{Theory issues}
\subsubsection{Experimental results}
\subsubsection{The case of the  $b\to ccd$ penguins}
\subsubsubsection{Theory issues}
\subsubsubsection{Experimental results}

\subsection{Measurement of the $B_s$ meson mixing phase}
\subsubsection{Theoretical predictions}
\subsubsection{Experimental results}

\subsection{Measurement of the angle \gg in tree dominated processes}
\subsubsection{Measurements of \gg in charged $B$ decays}
\subsubsubsection{The ADS technique}
\subsubsubsection{The GLW technique}
\subsubsubsection{Dalitz plot analyses}
\subsubsubsection{Combined results}
\subsubsection{Measurements of \gg in neutral $B$ decays}
\subsubsubsection{The ADS technique}
\subsubsubsection{The GLW technique}
\subsubsubsection{Dalitz plot analyses}
\subsubsubsection{Combined results}



==> symbols.tex <==
%%%%%  Uniformized symbols for the CKM 2008 book  %%%%%%%%%

\RequirePackage{xspace}
%%% last minute
\def\matrixelement#1#2#3{{\bra #1#2\ket#3}}
\def\Bzbar{\Bzb}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}
%\def\ev   {\ensuremath{\rm \,e\kern -0.08em V}}
%\def\kev  {\ensuremath{\rm \,ke\kern -0.08em V}} 
%\def\mev  {\ensuremath{\rm \,Me\kern -0.08em V}} 
%\def\gev  {\ensuremath{\rm \,Ge\kern -0.08em V}} 
%\def\gevc {\ensuremath{\rm \,Ge\kern -0.08em V\!/c}} 
%\def\gevc {\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c}} 
%\def\tev  {\ensuremath{\rm \,Te\kern -0.08em V}}
%\def\mevc {\ensuremath{\rm \,Me\kern -0.08em V\!/c}} 
%\def\mevc {\ensuremath{{\rm \,Me\kern -0.08em V\!/}c}} 
%\def\gevcc{\ensuremath{\rm \,Ge\kern -0.08em V\!/c^2}} 
%\def\mevcc{\ensuremath{\rm \,Me\kern -0.08em V\!/c^2}} 
%\def\gevcc{\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c^2}} 
%\def\mevcc{\ensuremath{{\rm \,Me\kern -0.08em V\!/}c^2}} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{{\rm \,km}}\xspace}
\def\m    {\ensuremath{{\rm \,m}}\xspace}
\def\cm   {\ensuremath{{\rm \,cm}}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{{\rm \,mm}}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
%\def\mum  {\ensuremath{{\rm \,\mum}}\xspace}
\def\mum  {\ensuremath{{\,\mu\rm m}}\xspace}%% mu meter 
%\def\muma {\ensuremath{\rm \,\mum}^2\xspace}
\def\muma       {\ensuremath{{\,\mu\rm m}^2}\xspace}
\def\nm   {\ensuremath{{\rm \,nm}}\xspace}
\def\fm   {\ensuremath{{\rm \,fm}}\xspace}
\def\nm         {\ensuremath{{\rm \,nm}}\xspace}   %% nanometer
%
\def\barn{\ensuremath{{\rm \,b}}\xspace}
\def\barnhyph{\ensuremath{{\rm -b}}\xspace}
\def\mbarn{\ensuremath{{\rm \,mb}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb         {\ensuremath{{\rm \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\rm \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}

%%\def\s{\ensuremath{\rm {\,s}}} %% second - this displays nothing  - why?
\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second - this works - jw 4/19
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond

 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   ARROWS        %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace} 
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
\def\num        {\ensuremath{\nu_\mu}\xspace}
\def\numb       {\ensuremath{\nub_\mu}\xspace}
\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}
\def\sbard {\ensuremath{\overline s d}\xspace}
\def\sdbar {\ensuremath{s\overline d}\xspace}

\def \mb  {\ensuremath{m_b}\xspace}
\def \mc  {\ensuremath{m_c}\xspace}
\def \mt  {\ensuremath{m_t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}
\def\rhoz  {\ensuremath{\rho^0}\xspace}
\def\rhop  {\ensuremath{\rho^+}\xspace}
\def\rhom  {\ensuremath{\rho^-}\xspace}
\def\rhopm  {\ensuremath{\rho^\pm}\xspace}
\def\rhomp  {\ensuremath{\rho^\mp}\xspace}
\def\rrz  {\ensuremath{\rho^0\rho^0}\xspace}
\def\rhorho  {\ensuremath{\rho^+\rho^-}\xspace}
\def\rhopi  {\ensuremath{\rho^+\pi^-}\xspace}

\def\Kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace} 
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace} 
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}
\def\Kone {\ensuremath{K^0_{\scriptscriptstyle 1}}\xspace}
\def\Ktwo {\ensuremath{K^0_{\scriptscriptstyle 2}}\xspace}
\def\Konetwo {\ensuremath{K^0_{\scriptscriptstyle 1,2}}\xspace}
\def\Ktwoone {\ensuremath{K^0_{\scriptscriptstyle 2,1}}\xspace}

\def\KLS {\ensuremath{K^0_{\scriptscriptstyle L,S}}\xspace}


\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsp      {\ensuremath{D^+_s}\xspace}
\def\Dsm      {\ensuremath{D^-_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}
\def\Dssp     {\ensuremath{D^{*+}_s}\xspace}
\def\Dssm     {\ensuremath{D^{*-}_s}\xspace}


\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}

%\def\chic1{\ensuremath{\chi_{c1}}}
%\def\chic2{\ensuremath{\chi_{c2}}}
%\def\chic3{\ensuremath{\chi_{c3}}}
\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} % dbm


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}

\def\Abar    {\kern 0.18em\overline{\kern -0.18em A}{}\xspace}
\def\BR         {{\ensuremath{\cal B}\xspace}}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}

% Define the \babar macro
\usepackage{relsize}
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}\xspace}

% Define LHCb
\def\lhcb {LHC{\em b\/}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   KINEMATICS    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ptot       {\mbox{$p$}\xspace}
\def\pxy        {\mbox{$p_T$}\xspace}
\def\pt         {\mbox{$p_T$}\xspace}
\def\mes        {\mbox{$m_{\rm ES}$}\xspace}
\def\mec        {\mbox{$m_{\rm EC}$}\xspace}
\def\Mbc        {\mbox{$M_{\rm bc}$}\xspace}
\def\DeltaE     {\mbox{$\Delta E$}\xspace}

\def\pbcm {\ensuremath{p^*_{\Bz}}\xspace}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   CKM           %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\eps{\varepsilon\xspace}
\def\epsK{\varepsilon_K\xspace}
\def \epsbarK {\bar\varepsilon_K\xspace}

\def\epsB{\varepsilon_B\xspace}
\def\epsp{\varepsilon^\prime_K\xspace}

\def\CP                {\ensuremath{C\!P}\xspace}
\def\CPT               {\ensuremath{C\!PT}\xspace} % Looks better without \!
\def\C       {\ensuremath{C}\xspace}
\def\P       {\ensuremath{P}\xspace}
\def\T       {\ensuremath{T}\xspace}

\def \SUthree {\ensuremath{{\rm SU}(3)_{\rm L}\times{\rm SU}(3)_{\rm R}}}
\def \SUtwo {\ensuremath{{\rm SU}(2)_{\rm L}\times{\rm SU}(2)_{\rm R}}}


\def\rhobar {\ensuremath{\overline \rho}\xspace}
\def\etabar {\ensuremath{\overline \eta}\xspace}

\def\Vud  {\ensuremath{|V_{ud}|}\xspace}
\def\Vcd  {\ensuremath{|V_{cd}|}\xspace}
\def\Vtd  {\ensuremath{|V_{td}|}\xspace}
\def\Vus  {\ensuremath{|V_{us}|}\xspace}
\def\Vcs  {\ensuremath{|V_{cs}|}\xspace}
\def\Vts  {\ensuremath{|V_{ts}|}\xspace}
\def\Vub  {\ensuremath{|V_{ub}|}\xspace}
\def\Vcb  {\ensuremath{|V_{cb}|}\xspace}
\def\Vtb  {\ensuremath{|V_{tb}|}\xspace}

%angles (important to use since they might change in time)

\def\aa{\ensuremath{\alpha}\xspace}
\def\bb{\ensuremath{\beta}\xspace}
\def\gm{\ensuremath{\gamma}\xspace}
\def\stwoa{\ensuremath{\sin\! 2 \alpha  }\xspace}
\def\stwob{\ensuremath{\sin\! 2 \beta   }\xspace}
\def\stwog{\ensuremath{\sin\! 2 \gamma  }\xspace}

%CP parameters
\def\Acp{\ensuremath{\mathcal{A}_{\CP}}\xspace}
\def\Scp{\ensuremath{\mathcal{S}_{\CP}}\xspace}
\def\Scpeff{\ensuremath{\mathcal{S}^{\rm eff}_{\CP}}\xspace}
\def\phioneeff{\ensuremath{\bb^{\rm eff}}\xspace}

% tagging
\def\mistag{\ensuremath{w}\xspace}
\def\dilution{\ensuremath{\cal D}\xspace}
\def\deltaz{\ensuremath{{\rm \Delta}z}\xspace}
\def\deltat{\ensuremath{{\rm \Delta}t}\xspace}
\def\deltamd{\ensuremath{{\rm \Delta}m_d}\xspace}
\def\deltam{\ensuremath{{\rm \Delta}m}\xspace}
\def\deltamK{\ensuremath{{\rm \Delta}m_K}\xspace}
\def\Btag {\ensuremath{B_{\rm tag}}}

% Branching fraction
\def\BR         {{\ensuremath{\cal B}\xspace}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   Lattice Paramters%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\fsubd}{\ensuremath{f_D}}\xspace
\newcommand{\fds}{\ensuremath{f_{D_s}}\xspace}
\newcommand{\fsubb}{\ensuremath{f_B}\xspace}
\newcommand{\fbd}{\ensuremath{f_{B_d}}\xspace}
\newcommand{\fbs}{\ensuremath{f_{B_s}}\xspace}
\newcommand{\bsubb}{\ensuremath{B_B}\xspace}
\newcommand{\bbd}{\ensuremath{B_{B_d}}\xspace}
\newcommand{\bbs}{\ensuremath{B_{B_s}}\xspace}
\newcommand{\rgbb}{\ensuremath{\hat{B}_B}\xspace}
\newcommand{\rgbbd}{\ensuremath{\hat{B}_{B_d}}\xspace}
\newcommand{\rgbbs}{\ensuremath{\hat{B}_{B_s}}\xspace}
\newcommand{\rgbk}{\ensuremath{\hat{B}_K}\xspace}
\newcommand{\lqcd}{\ensuremath{\Lambda_{\mathrm{QCD}}}\xspace}

%\def\subsubsubsection   {\subsubsection*}


%%%%%%%%%%%%%%%%%%%% Cabibbo 

% Macros: Variables and mathematical expressions

\newcommand{\Rs}{\ensuremath{R_S}}
\newcommand{\Rl}{\ensuremath{R_L}}
\newcommand{\Rsg}{\ensuremath{R_{S,\gamma}}}

\def\ifm#1{\relax\ifmmode#1\else$#1$\fi}
\def\DAF{DA\char8NE}    \def\vv{\vphantom{H^I_I}}
\def\x{\ifm{\times}}   \def\pt#1,#2,{\ifm{#1\x10^{#2}}}
\def\up#1{\ifm{^{#1}}}   \def\dn#1{\ifm{_{#1}}}  \def\plm{\ifm{\,\pm}\,}
\def\ab{\ifm{\sim}}   \def\deg{\ifm{^\circ}}
\def\gam{\ifm{\gamma}}  \def\eps{\ifm{\epsilon}}
%\def\to{\ifm{\rightarrow}}
\def\kl{\ifm{K_L}}   \def\ks{\ifm{K_S}}
\def\eiii{\ifm{\pi^\pm e^\mp\nu}}
\def\keiii{\ifm{K_{e3}}}
\def\muiii{\ifm{\pi^\pm \mu^\mp\nu}}
\def\kmuiii{\ifm{K_{\mu3}}}
\def\pio{\ifm{\pi^0\pi^0}}
\def\po{\ifm{\pi^0}}
\def\pic{\ifm{\pi^+\pi^-}}
\def\K{\ifm{K}}
\def\rmk{\rm\kern.5mm }
\def\f{\ifm{\phi}}
\def\eqq#1{(\ref{#1})}
\def\eq#1{Eq.~(\ref{#1})}
\def\GAML{\ifm{\Gamma_L}}   \def\minus{$-$}
\def\GAMS{\ifm{\Gamma_S}}
\def\ko{\ifm{K^0\vphantom{\overline K {}^0}}}
\def\kob{\ifm{\overline K {}^0}}
\def\figb#1;#2;{\parbox{#2cm}{\epsfig{file=#1.eps,width=#2cm}}}
 \def\O{{\cal O}}

\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}

\newcommand{\be}{\begin{equation}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\no}{\nonumber}
\newcommand{\nn}{\nonumber}
\newcommand{\dis}{\displaystyle}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cA}{\mathcal{A}}
\def\Gno{\ifm{\Gamma_{\ko}}}
\def\Gnb{\ifm{\Gamma_{\kob}}}
\def\Mno{\ifm{m_{\ko}}}
\def\Mnb{\ifm{m_{\kob}}}
\def\Re{{\rm Re}}
\def\Im{{\rm Im}}


\newcommand{\Ref}[1]{Ref.~\cite{#1}}
\newcommand{\Refs}[1]{Refs.~\cite{#1}}
\newcommand{\andRef}[1]{and~\cite{#1}}
\newcommand{\Fig}[1]{Fig.~\ref{#1}}
\newcommand{\Sec}[1]{Sec.~\ref{#1}}
\newcommand{\Tab}[1]{Tab.~\ref{#1}}
\newcommand{\Eq}[1]{Eq.~(\ref{#1})}
%\newcommand{\etal}{et al.}

\newcommand{\BRT}[1]{\ensuremath{{\cal B}(#1)}}
\newcommand{\bra}[1]{\ensuremath{\left<#1\right|}}
\newcommand{\ket}[1]{\ensuremath{\left|#1\right>}}
\newcommand{\mean}[1]{\ensuremath{\left<#1\right>}}
\newcommand{\order}[1]{\ensuremath{\mathcal{O}(#1)}}
\newcommand{\SN}[2]{\ensuremath{#1\times10^{#2}}}
\renewcommand{\vec}[1]{\ensuremath{\mathbf{#1}}}

\newcommand{\tr}{\ensuremath{^{\rm T}}}
\newcommand{\inv}{\ensuremath{^{-1}}}
\newcommand{\stat}{\ensuremath{_\mathrm{st}}}
\newcommand{\syst}{\ensuremath{_\mathrm{sy}}}
\newcommand{\theo}{\ensuremath{_\mathrm{th}}}
\newcommand{\ext}{\ensuremath{_\mathrm{ext}}}
\newcommand{\cross}{\ensuremath{\mathbf{\times}}}
\renewcommand{\dot}{\ensuremath{\mathbf{\cdot}}}
%\newcommand{\Vud}{\ensuremath{|V_{ud}|}}
%\newcommand{\Vus}{\ensuremath{|V_{us}|}}
%\newcommand{\Vub}{\ensuremath{|V_{ub}|}}
\newcommand{\Vusf}{\ensuremath{|V_{us}|f_+(0)}}
\newcommand{\RepsK}{\ensuremath{{\rm Re}(\varepsilon_K)}}
\newcommand{\Reps}{\ensuremath{{\rm Re}\:\epsilon'/\epsilon}}
\newcommand{\Repsp}{\ensuremath{Re(\epsp/\epsK)}}
\newcommand{\Impsp}{\ensuremath{Im(\epsp/\epsK)}}
\newcommand{\Imdelta}{\ensuremath{Im(\delta)}}

\newcommand{\DeKP}{(m^2_K-m^2_\pi)}
\newcommand{\SigKP}{(m^2_K+m^2_\pi)}
\newcommand{\fp}{f_+(0)}
%\newcommand{\gev}{{\rm GeV}}
%\newcommand{\mev}{{\rm MeV}}
%\newcommand{\text}{\rm}
%\newcommand{\vus}{\vert V_{us}\vert}
\newcommand{\fplust}{\mbox{$\hat{f}_+(t)$}}
\newcommand{\fminust}{\mbox{$f_-(t)$}}
\newcommand{\fzerot}{\mbox{$\hat{f}_0(t)$}}



%%%%%%%%%%%%%%%  New definitions by Towner-Plaster 

\def\bea {\begin{eqnarray}}
\def\eea {\end{eqnarray}}
\def\be {\begin{equation}}
\def\ben{\begin{enumerate}}
\def\een{\end{enumerate}}
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}
\def\ie{{\it i.e.}\ }
\def\viz{{\it viz.}\ }
\def\eg{{\it e.g.}\ }
\def\etal{{\it et al.}\ }
\def\del{\partial}
\def\O{{\mathcal{O}}}
\def\F{{\mathcal{F}}}
\def\prl {Phys. Rev. Lett.\ }
\def\pl {Phys. Lett.\ }
\def\pr {Phys. Rev.\ }
\def\np {Nucl. Phys.\ }
\def\gV{g_{\mbox{\tiny V}}}
\def\gA{g_{\mbox{\tiny A}}}
\def\fM{f_{\mbox{\tiny M}}}
\def\fT{f_{\mbox{\tiny T}}}
\def\fS{f_{\mbox{\tiny S}}}
\def\fP{f_{\mbox{\tiny P}}}
\def\MN{M_{\mbox{\tiny N}}}
\def\MW{M_{\mbox{\tiny W}}}
\def\GV{G_{\mbox{\tiny V}}}
\def\GF{G_{\mbox{\tiny F}}}
\def\DRV{\Delta_{\mbox{\tiny R}}^{\mbox{\tiny V}}}
\def\mA{m_{\mbox{\tiny A}}}
\def\mZ{m_{\mbox{\tiny Z}}}
\def\dbar{\mid \! \mid }
\def\hyphen{{\mbox{-}}}
\def\hhphen{\, {\mbox{--}}}
\newcommand{\sfrac}[2]{\mbox{\small{$\frac{#1}{#2}$}}}

\newcounter{saveeqn}
\newcommand{\alpheqn}{\setcounter{saveeqn}{\value{equation}}%
  \stepcounter{saveeqn}\setcounter{equation}{0}%
  \renewcommand{\theequation}{\mbox{\arabic{saveeqn}\alph{equation}}}}
\newcommand{\reseteqn}{\setcounter{equation}{\value{saveeqn}}%
  \renewcommand{\theequation}{\arabic{equation}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% first used in Bs mixing phase phi_s section (lifemix-phi-s.tex)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
\newcommand{\BsJphi}{\Bs \to \jpsi\phi}
\newcommand{\betas}{\ensuremath{\beta_{s}^{J/\psi\phi}}}        % the actual phase that is measured in psi phi Bs decays
\newcommand{\betasSM}{\ensuremath{\beta_{s}^{\mathrm{SM}}}}     % the SM value of the Bspsiphi phase
\newcommand{\betasNP}{\ensuremath{\beta_{s}^{\mathrm{NP}}}}     % the NP contribution to the Bspisphi phase

\newcommand{\phis}{\ensuremath{\phi_{s}^{J/\psi\phi}}}          % quantities in terms of phi (inteas of beta)
\newcommand{\phisSM}{\ensuremath{\phi_{s}^{\mathrm{SM}}}}
\newcommand{\phisNP}{\ensuremath{\phi_{s}^{\mathrm{NP}}}}

\newcommand{\DGNP}{\ensuremath{\Delta\Gamma^{\mathrm{NP}}}}
\newcommand{\DGSM}{\ensuremath{\Delta\Gamma^{\mathrm{SM}}}}
\newcommand{\BdJKst}{\Bz \to \jpsi\Kstar}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% first used by coleman for D0 mixing (lifemix-charm.tex)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\order{{\ensuremath{\cal O}}\xspace}
\def\DztoKPi    {\ensuremath{\Dz \to K\pi}\xspace}
\def\Dztokpi    {\ensuremath{\Dz \to K^{-}\pi^{+}}\xspace}
\def\DztokpiWS  {\ensuremath{\Dz \to K^{+}\pi^{-}}\xspace}
\def\DzbtokpiWS {\ensuremath{\Dzb \to K^{-}\pi^{+}}\xspace}
\def\Dzbtokpi   {\ensuremath{\Dzb \to K^{+}\pi^{-}}\xspace}
\def\Rdcs       {\ensuremath{R_{\rm D}}\xspace}
\def\Dstp       {\ensuremath{D^{*+}}}
\def\pisoft     {\ensuremath{\pi_{\rm s}}\xspace}
\def\Tws        {\ensuremath{T_{\rm WS}(t)}}
\def\yPrime     {\ensuremath{y^{\prime}}\xspace}
\def\xPrimeSq   {\ensuremath{{x^{\prime}}^2}\xspace}
\def\yPrimeSq   {\ensuremath{{y^{\prime}}^2}\xspace}
\def\xPrime     {\ensuremath{x^{\prime}}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\yCP        {\ensuremath{y_{C\!P}}\xspace}
\def\pippim     {\ensuremath{\pi^{+}\pi^{-}}\xspace}
\def\Kmpip      {\ensuremath{K^{-}\pi^{+}}\xspace}
\def\KmKp       {\ensuremath{K^{-}K^{+}}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% first used by martin for cp violation in charmonium (lifemix-bccs.tex)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\effectiveeta{0.504 \pm 0.033}

\def\ifb       {\ensuremath{ { fb^{-1} }}}

\newcommand\etap {\ensuremath{\eta^\prime}}
\def\CPV{\ensuremath{CPV}}
\def\ifb{\ensuremath{\mathrm{fb^{-1}}}}
\def\iab{\ensuremath{\mathrm{ab^{-1}}}}
\def\D{\ensuremath{D}}
\def\ptrue{\ensuremath{f_L}}
\newcommand\sgline{\noalign{\vskip 0.10truecm\hrule\vskip 0.10truecm}}
\newcommand\sgdline{\noalign{\vskip 0.10truecm\hrule\vskip 0.05truecm\hrule\vskip 0.10truecm}}

\def\etal{{\em et al}}


\def\btoccbars{\ensuremath{\b\rightarrow\c\cbar\s}}
\def\ctwob{\ensuremath{\cos\! 2 \beta   }\xspace}

\newcommand{\bflav}{\ensuremath{\B_{{\rm flav}}}}

\def\Dzero{D{\cal{0}}}


%%%%%%%%%%%%  U.T. FITS  %%%%%%%%%%%
\newcommand{\noi}{\noindent}
\newcommand{\nl}{\newline}
\newcommand{\tb}{\textbullet}
\renewcommand{\topfraction}{1}
\renewcommand{\bottomfraction}{1}
\renewcommand{\textfraction}{0}
\renewcommand{\topfraction}{1}
\renewcommand{\floatpagefraction}{1}
\newcommand{\calO}{{\mathcal O}}
\def \utfit {{\bf UT}{\it fit}~}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Additional symbols for Hadron Collider and experimental primer
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\eD} {\ensuremath{\varepsilon{\mathcal D}^2}} % used
\newcommand{\ptrel} {\ensuremath{p_T^{\rm rel}}}  %used
\newcommand{\bsd}      {\Bsb\to \Ds\pi^-}             % used 
\newcommand{\bsdppp}   {\Bsb\to \Ds \pi^+\pi^-\pi^+}  % used
\newcommand{\bud}      {\Bub\to D^0\pi^-}  %used
\newcommand{\bdd}      {\Bzb\to D^+\pi^-}  %used
\newcommand{\ppbar}  {\ensuremath{p \overline p}} %used
\newcommand{\ase}[2]{\ensuremath{^{~+ #1}_{~- #2}}} %used
\newcommand{\BsBsbar}{\ensuremath{B^0_s}-\ensuremath{\overline{B}^0_s}} %used
\newcommand{\DeltaR} {\ensuremath{\delta R}} %used

